Examining Untempered Social Media: Analyzing Cascades of Polarized Conversations

Online social media, periodically serves as a platform for cascading polarizing topics of conversation. The inherent community structure present in online social networks (homophily) and the advent of fringe outlets like Gab have created online "echo chambers" that amplify the effects of polarization, which fuels detrimental behavior. Recently, in October 2018, Gab made headlines when it was revealed that Robert Bowers, the individual behind the Pittsburgh Synagogue massacre, was an active member of this social media site and used it to express his anti-Semitic views and discuss conspiracy theories. Thus to address the need of automated data-driven analyses of such fringe outlets, this research proposes novel methods to discover topics that are prevalent in Gab and how they cascade within the network. Specifically, using approximately 34 million posts, and 3.7 million cascading conversation threads with close to 300k users; we demonstrate that there are essentially five cascading patterns that manifest in Gab and the most "viral" ones begin with an echo-chamber pattern and grow out to the entire network. Also, we empirically show, through two models viz. Susceptible-Infected and Bass, how the cascades structurally evolve from one of the five patterns to the other based on the topic of the conversation with upto 84% accuracy.

==> evolution.tex <==
%\section{Evolution of cascades}


==> foundation.tex <==
\section{Foundational Data Analysis}

\subsection{Dataset Description}
\label{sect:data_desc}
Gab.ai is a new social networking media, founded in 2016, to share information and views with other users in the forum. Even though the description of the forum looks very similar to other social networks like Twitter, Gab.ai is known for individual liberty and free speech in online\footnote{https://gab.ai/}. Further, Gab.ai has strong restriction policies on posts and users promoting pornography, terrorism and violence. Users of gab.ai can share information via \textit{posts}, \textit{post replies}, \textit{quotes}(Sharing and commenting on a post) and \textit{post shares}. 

The data that we collected comprise of around \textbf{14M posts} from about \textbf{175,000 users} covering the date range from August 2016 to September 2018. We collected all details of each post or comment like \textit{message body, created at, attachments, like-dislike-repost-reply counts, conversation threads, category} and \textit{user details} attached with these messages like \textit{id, username, friends-followers count} and \textit{screen name}. Apart from collecting all textual data, we also collected social network(\textit{friends} and \textit{followers}) of  \textbf{390,889} public users in Gab.ai.

\subsection{Simple timeseries analysis}


\subsection{Simple topic modelling}


\subsection{Simple social network analysis}
With the availability of social(friends/followers) network of the Gab.ai, we analyze mostly connected users and their behaviour in Gab.ai. The social network that we collected is a single component network and it contains 390,889 nodes and 10.7M edges. Figure~\ref{fig:degree_dist} depicts the degree distribution of the social network of Gab.ai. For a very simple influence measure, we consider users with very large number of connections($in-degree>=1000$), compare their connectivity patterns in the social network and behaviour in Gab.ai. We found that \textbf{632} users fall under this category and more than \textbf{$46\%$} of the total social network nodes follow these users. We also analyzed the ego-network of these users and found that this ego-net covers around \textbf{9M} edges(approximately $85\%$ of total edges in the social network). 

\begin{figure}
\centering
\includegraphics[scale=0.5]{follower_net_degree_dist.png}
\caption{Degree distribution of the follower network of Gab.ai} \label{fig:degree_dist}
\end{figure}

==> results.tex <==
\section{Case Study}

\begin{figure}
\centering
\includegraphics[scale=0.35]{domain.png}
\caption{Wordcloud of most frequently occurring URL domain names in Gab posts. This represents the domination of alt-right domain names in Gab eventhough there exists few popular neutral news domains.} \label{fig:domains}
\end{figure}

Our experiments are based on the existence of alternative/conservative and mainstream news media articles in Gab posts. Our collection of conservative and liberal new media is from "ad fontes media"\footnote{https://www.adfontesmedia.com/}, which gives a broad overview of URL domains based on their unfair and genuine content interpretations to the public. Based on this collection, we give Figure~\ref{fig:domains}, which shows that Gab users follow and share more conservative news domains than mainstream news articles. We also give the distribution of maximum number of posts with mainstream and alternative news domains being used alternatively over time during shock events. Figure~\ref{fig:oscillation} gives such an oscillation of news media forum being popular during the Charlottesville protest in 2017.

\begin{figure}
\centering
\includegraphics[scale=0.35]{oscillation.png}
\caption{Evidence of alternative and mainstream news media taking turns in gaining traction over time via posts in Gab during the shock event - Charlottesville protest(12 Aug 2017)} \label{fig:oscillation}
\end{figure}

\subsection{Case study 1: Charlottesville protest}
For the Charlottesville protest event, we only consider posts that appeared in Gab.com on the protest day(12 Aug 2017). Gab evidence conversations of blame and accusation on this day as the support for the alt-right protesters moved from Emancipation Park to the online spaces of Gab.ai. Until around 2pm on the day of the protest, majority of discussions are consistently painting the anti-fascist counter protesters as violent while the alt-right demonstrators are maintaining peace and respect. During the next hour between 2pm-3pm the first set of news articles begin to spread about a car driving into a crowd of protesters. Discussions are primarily based on physical observations as news consisting of images and videos is shared on the platform is focused mostly around sharing basic facts around what happened. During the second hour after the attack the discussions move from talking about the physical events into comments about the meaning of the attack and who is to blame for it. Soon the narrations in Gab focus over a domestic terrorist, who was not a trump supporter in attempts to distance the alt-right movement and their leader from any negative attention. Later in the hour Trump appears on national TV and blames "many sides" for the violence. During the fourth hour (4pm-5pm) users revisit physical events of the day and construct evidence for various conspiracy theories. One theory that begins to take hold is that the driver \lq s airbag did not deploy and it must have been premeditated. Or that police had the wrong perpetrator of the attack in custody. During the fifth hour (5pm-6pm) false narratives continue to spread as the community process new information about the attack. Rumors about the real perpetrator of the attack result in the doxing of an unrelated person who was found to have a picture of a similar looking dodge challenger on their Facebook profile. Worries spread about the possible use of the hate crime as justification to silence the alt-right \lq s ability to speak without censorship. News of a helicopter crash begin to spread and is immediately adopted into conspiracy theories connecting the two events as part of a larger organized plan. Throughout the rest of the day doxing continues of a falsely accused "open borders druggie" as being the perpetrator of the attack. And the prevailing narrative expands into a larger discussion around the importance of free speech and how the anti-fascist counter-protestors are not receiving blame they deserve from the mainstream media.

\begin{figure*}
\centering
\includegraphics[scale=0.30]{char.png}
\caption{Timeline of events during the Charlottesville protest and the corresponding online discussions in Gab during the shock event} \label{fig:charlleston_study}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[scale=0.30]{pittsburgh.png}
\caption{Events timeline and online discussions in Gab in effect of mainstream news articles during the Pittsburgh synagauge shooting.} \label{fig:pittsburgh_study}
\end{figure*}

\subsection{Case study 2: Pittsburgh synagauge shooting}
Detected subevents for the day of October 27th were analyzed for evolving narratives. 
A clear narrative emerged on how discussions around the breaking news evolve across the day.
Within the first hour when the news broke on Gab links were posted to news about the shooting. 9/28 of these posts contained hate speech. The first alternative narrative begins to appear two hours after the shooting news broke, as the shooting being planned event in a larger conspiracy by President Donald Trump\lq s political opponents to gain political power before the November 6th election. 
Example: https://www.puppetstringnews.com/blog/8-dead-3-cops-shot-at-pittsburgh-jewish-synagogue-shooter-yelled-all-jews-must-die ( puppetstring news has been shared 15,313 on gab)
During the third hour the conversation turned to discussions around false flag operations and the alt-right conspiracy theory known as "Qanon". An alt-right support march known as "\#WalkAway" was happening during the afternoon and news of this rally was shadowed by the release of news regarding the shooting event. Providing a motive to the conspiracy that the shooting was planned.  The narratives around the shooting even begin to coalesce around the four and fifth hour with the publication of infowar’s live stream painting the shooting as "the latest move by the Deep State to sow civil unrest and effect the historic upcoming midterm election": https://www.infowars.com/breaking-alex-jones-goes-live-to-respond-to-terrorist-attack-on-pittsburgh-synagogue-the-deep-state-has-played-its-terror-card/  (Link was posted at 1:30central time and was shared 36 times during the day)

Five hours after the shooting the form of the media shared changes to become more long form, youtube videos of analysis and commentary. Blog articles explaining a range of conspiracies involving a deepstate plot to attack the second amendment or to try to limit free speech, or to try to embarrass President trump. Our analysis shows the collective sense making~\cite{meyersohn1969improvised} as people begin to provide explanations that align with their sense of reality in order to reduce anxiety and provide a sense of understanding and control of the news~\cite{van2015influence, mandik2007shit}.


\begin{figure}[!ht]
	\centering	
		\subfloat[Figure a: Average popularity of posts at all branches in different cascades\label{fig:branch_popularity}]{\includegraphics[scale=0.23]{casestudy_2.png}}	
	
		\qquad	
	
		\subfloat[Figure b: Average popularity of posts at root level in different cascades\label{fig:root_popularity}]{\includegraphics[scale=0.23]{casestudy_4.png}}


		\caption{Average popularity of posts at root level and other levels in different cascade types for twot events}
		\label{fig:event_popularity}
\end{figure}

In addition to observing information mutation between news media and posts, we give an overview of popularity scores for posts that appeared on these event days. For Charlottesville protest we extracted \textbf{27,031} cascades and for Pittsburgh event we extracted \textbf{20,083} cascades. In Figure~\ref{fig:event_popularity}, me give plots for the distribution of popularity scores for posts that created cascades during these events(Figure~\ref{fig:root_popularity}) and also to posts that are replies and quotes to root nodes(Figure~\ref{fig:branch_popularity}). From these figures, we note that root nodes have higher popularity scores compared to other posts during shock events and also that cascade type E takes higher popularity measures at root level compared to other posts. 
